IterativeCUR: Large Rank-Adaptive Approximation From a Small Recycled Sketch

The computation of accurate low-rank matrix approximations is central to improving the scalability of various techniques in machine learning, uncertainty quantification, and control. Traditionally, low-rank approximations are constructed using SVD-based approaches such as truncated SVD or Randomized SVD. Although these SVD approaches---especially Randomized SVD---have proven to be very computationally efficient, other low-rank approximation methods can offer even greater performance. One such approach is the CUR decomposition, which forms a low-rank approximation using direct row and column subsets of a matrix. Because CUR uses direct matrix subsets, it is also often better able to preserve native matrix structures like sparsity or non-negativity than SVD-based approaches and can facilitate data interpretation in many contexts. This paper introduces IterativeCUR, which draws on previous work in randomized numerical linear algebra to build a new algorithm that is highly competitive compared to prior work. IterativeCUR is adaptive in the sense that it takes as an input parameter the desired tolerance $\epsilon$ and outputs (with arbitrarily high probability) an approximation of error bounded by $\epsilon$, rather than requiring an a priori guess of the numerical rank. IterativeCUR typically runs significantly faster than both existing CUR algorithms and techniques such as Randomized SVD. Its asymptotic complexity is $\mathcal{O}(mn + (m+n)r^2)$ for an $m\times n$ matrix of output rank $r$. IterativeCUR relies on a single small sketch from the matrix that is successively downdated as the algorithm proceeds. We demonstrate through extensive experiments that IterativeCUR achieves up to $4\times$ speed-up over state-of-the-art pivoting-on-sketch approaches with no loss of accuracy, and up to $40\times$ speed-up over rank-adaptive randomized SVD approaches.

==> plots/block_size/TSOPF.tex <==
\begin{tikzpicture}[scale = \boxplotscale]
    \newcommand{\matname}{TSOPF}
    \newcommand{\Matname}{\textsc{TSOPF} }
    \pgfplotstableread[col sep=comma]{./csvs/block_size/\matname_accuracy.csv}\accdata
    \pgfplotstableread[col sep=comma]{./csvs/block_size/\matname_time.csv}\timedata
    
    \begin{axis}[
        name = axis1,
        ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Accuracy for \Matname Across Block Sizes},
        %ymode = log,
        ymajorgrids,
        legend pos = north east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[bs5_line]table[x = n_cols, y = bs_5]\accdata;
        \addplot[bs50_line]table[x = n_cols, y = bs_50]\accdata;
        \addplot[bs100_line]table[x = n_cols, y = bs_100]\accdata;
        \addplot[bs500_line]table[x = n_cols, y = bs_500]\accdata;
        \legend{5, 50, 100, 500};
    \end{axis}
    \begin{axis}[
        name = axis2,
        at={(axis1.outer north east)},
        anchor=outer north west,
        ylabel = {Time (Seconds)},
        xlabel = {Rank of Approximation},
        title = {Time for \Matname Across Block Sizes},
        %ymode = log,
        ymajorgrids,
        legend pos = south east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[bs5_line]table[x = n_cols, y = bs_5]\timedata;
        \addplot[bs50_line]table[x = n_cols, y = bs_50]\timedata;
        \addplot[bs100_line]table[x = n_cols, y = bs_100]\timedata;
        \addplot[bs500_line]table[x = n_cols, y = bs_500]\timedata;
        %\legend{\svds, \curs, \icurl};
    \end{axis}
\end{tikzpicture}

==> plots/block_size/randsvd.tex <==
\begin{tikzpicture}[scale = \boxplotscale]
    \newcommand{\matname}{RandSVD}
    \newcommand{\Matname}{\textsc{RandSVD} }
    \pgfplotstableread[col sep=comma]{./csvs/block_size/\matname_accuracy.csv}\accdata
    \pgfplotstableread[col sep=comma]{./csvs/block_size/\matname_time.csv}\timedata
       \begin{axis}[
        name = axis1,
        ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Accuracy for \Matname Across Block Sizes},
        %ymode = log,
        ymajorgrids,
        legend pos = north east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[bs5_line]table[x = n_cols, y = bs_5]\accdata;
        \addplot[bs50_line]table[x = n_cols, y = bs_50]\accdata;
        \addplot[bs100_line]table[x = n_cols, y = bs_100]\accdata;
        \addplot[bs500_line]table[x = n_cols, y = bs_500]\accdata;
        \legend{5, 50, 100, 500};
    \end{axis}
    \begin{axis}[
        name = axis2,
        at={(axis1.outer north east)},
        anchor=outer north west,
        ylabel = {Time (Seconds)},
        xlabel = {Rank of Approximation},
        title = {Time for \Matname Across Block Sizes},
        %ymode = log,
        ymajorgrids,
        legend pos = south east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[bs5_line]table[x = n_cols, y = bs_5]\timedata;
        \addplot[bs50_line]table[x = n_cols, y = bs_50]\timedata;
        \addplot[bs100_line]table[x = n_cols, y = bs_100]\timedata;
        \addplot[bs500_line]table[x = n_cols, y = bs_500]\timedata;
        %\legend{\svds, \curs, \icurl};
    \end{axis}
\end{tikzpicture}

==> plots/kahan/kahan_median_acc.tex <==
\begin{tikzpicture}[scale = \boxplotscale]
    \newcommand{\matname}{ct20stif}
    \newcommand{\Matname}{Ct20Stif}
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_LUPP_iterative_cur.csv}\IluppO
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_10_LUPP_iterative_cur.csv}\IluppTe
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_20_LUPP_iterative_cur.csv}\IluppTw
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_40_LUPP_iterative_cur.csv}\IluppFe
     \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_LUPP_sketch_cur.csv}\sluppO
     
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_QRPP_iterative_cur.csv}\IqrcpO
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_10_QRPP_iterative_cur.csv}\IqrcpTe
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_20_QRPP_iterative_cur.csv}\IqrcpTw
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_40_QRPP_iterative_cur.csv}\IqrcpFe
     \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_QRPP_sketch_cur.csv}\sqrcpO
     
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_OSPP_iterative_cur.csv}\IosO
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_10_OSPP_iterative_cur.csv}\IosTe
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_20_OSPP_iterative_cur.csv}\IosTw
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_40_OSPP_iterative_cur.csv}\IosFe
     \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_OS_sketch_cur.csv}\sosO
       \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_svds.csv}\svdsO
    \begin{axis}[
        name = axis1,
        ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Median Accuracy Block Size 1},
        ymode = log,
        ymajorgrids,
        legend pos = south east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[sqr_line]table[x = n_rows, y = median_acc]\sqrcpO;
        \addplot[scur_line]table[x = n_rows, y = median_acc]\sluppO;
        \addplot[sos_line]table[x = n_rows, y = median_acc]\sosO;
        \addplot[svds_line]table[x = n_rows, y = median_acc]\svdsO;
        \addplot[icur_line]table[x = n_rows, y = median_acc]\IluppO;
        \addplot[qr_line]table[x = n_rows, y = median_acc]\IqrcpO;
        \addplot[os_line]table[x = n_rows, y = median_acc]\IosO;
        
        %\legend{\svds, \curs, \icurl};
    \end{axis}
    
    \begin{axis}[
        name = axis2,
        at={(axis1.outer north east)},
        anchor=outer north west,
         ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Median Accuracy Block Size 10},
        ymode = log,
        ymajorgrids,
        legend pos = south east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
      \addplot[sqr_line]table[x = n_rows, y = median_acc]\sqrcpO;
        \addplot[scur_line]table[x = n_rows, y = median_acc]\sluppO;
        \addplot[sos_line]table[x = n_rows, y = median_acc]\sosO;
        \addplot[svds_line]table[x = n_rows, y = median_acc]\svdsO;
        \addplot[icur_line]table[x = n_rows, y = median_acc]\IluppTe;
        \addplot[qr_line]table[x = n_rows, y = median_acc]\IqrcpTe;
        \addplot[os_line]table[x = n_rows, y = median_acc]\IosTe;
        %\legend{\svds, \curs, \icurl};
    \end{axis}

        \begin{axis}[
        name = axis3,
        at={(axis1.outer south west)},
        anchor=outer north west,
         ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Median Accuracy Block Size 20},
        ymode = log,
        ymajorgrids,
        legend pos = south east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[sqr_line]table[x = n_rows, y = median_acc]\sqrcpO;
        \addplot[scur_line]table[x = n_rows, y = median_acc]\sluppO;
        \addplot[sos_line]table[x = n_rows, y = median_acc]\sosO;
        \addplot[svds_line]table[x = n_rows, y = median_acc]\svdsO;
        \addplot[icur_line]table[x = n_rows, y = median_acc]\IluppTw;
        \addplot[qr_line]table[x = n_rows, y = median_acc]\IqrcpTw;
        \addplot[os_line]table[x = n_rows, y = median_acc]\IosTw;
        %\legend{\svds, \curs, \icurl};
    \end{axis}

            \begin{axis}[
        at={(axis3.outer north east)},
        anchor=outer north west,
         ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Median Accuracy Block Size 40},
        ymode = log,
        ymajorgrids,
        legend pos = south east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[sqr_line]table[x = n_rows, y = median_acc]\sqrcpO;
        \addplot[scur_line]table[x = n_rows, y = median_acc]\sluppO;
        \addplot[sos_line]table[x = n_rows, y = median_acc]\sosO;
        \addplot[svds_line]table[x = n_rows, y = median_acc]\svdsO;
        \addplot[icur_line]table[x = n_rows, y = median_acc]\IluppFe;
        \addplot[qr_line]table[x = n_rows, y = median_acc]\IqrcpFe;
        \addplot[os_line]table[x = n_rows, y = median_acc]\IosFe;
        %\legend{\svds, \curs, \icurl};
    \end{axis}
\end{tikzpicture}

==> plots/kahan/kahan_var_acc.tex <==
\begin{tikzpicture}[scale = \boxplotscale]
    \newcommand{\matname}{ct20stif}
    \newcommand{\Matname}{Ct20Stif}
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_LUPP_iterative_cur.csv}\IluppO
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_10_LUPP_iterative_cur.csv}\IluppTe
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_20_LUPP_iterative_cur.csv}\IluppTw
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_40_LUPP_iterative_cur.csv}\IluppFe
     \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_LUPP_sketch_cur.csv}\sluppO
     
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_QRPP_iterative_cur.csv}\IqrcpO
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_10_QRPP_iterative_cur.csv}\IqrcpTe
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_20_QRPP_iterative_cur.csv}\IqrcpTw
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_40_QRPP_iterative_cur.csv}\IqrcpFe
     \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_QRPP_sketch_cur.csv}\sqrcpO
     
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_OSPP_iterative_cur.csv}\IosO
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_10_OSPP_iterative_cur.csv}\IosTe
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_20_OSPP_iterative_cur.csv}\IosTw
    \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_40_OSPP_iterative_cur.csv}\IosFe
     \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_OS_sketch_cur.csv}\sosO
       \pgfplotstableread[col sep=comma]{./csvs/kahan/kahan_500_1_svds.csv}\svdsO
    \begin{axis}[
        name = axis1,
        ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Median Accuracy Block Size 1},
        ymode = log,
        ymajorgrids,
        legend pos = south east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[sqr_line]table[x = n_rows, y = var_acc]\sqrcpO;
        \addplot[scur_line]table[x = n_rows, y = var_acc]\sluppO;
        \addplot[sos_line]table[x = n_rows, y = var_acc]\sosO;
        \addplot[icur_line]table[x = n_rows, y = var_acc]\IluppO;
        \addplot[qr_line]table[x = n_rows, y = var_acc]\IqrcpO;
        \addplot[os_line]table[x = n_rows, y = var_acc]\IosO;
        
        %\legend{\svds, \curs, \icurl};
    \end{axis}
    
    \begin{axis}[
        name = axis2,
        at={(axis1.outer north east)},
        anchor=outer north west,
         ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Median Accuracy Block Size 10},
        ymode = log,
        ymajorgrids,
        legend pos = south east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
      \addplot[sqr_line]table[x = n_rows, y = var_acc]\sqrcpO;
        \addplot[scur_line]table[x = n_rows, y = var_acc]\sluppO;
        \addplot[sos_line]table[x = n_rows, y = var_acc]\sosO;
        \addplot[icur_line]table[x = n_rows, y = var_acc]\IluppTe;
        \addplot[qr_line]table[x = n_rows, y = var_acc]\IqrcpTe;
        \addplot[os_line]table[x = n_rows, y = var_acc]\IosTe;
        %\legend{\svds, \curs, \icurl};
    \end{axis}

        \begin{axis}[
        name = axis3,
        at={(axis1.outer south west)},
        anchor=outer north west,
         ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Median Accuracy Block Size 20},
        ymode = log,
        ymajorgrids,
        legend pos = south east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[sqr_line]table[x = n_rows, y = var_acc]\sqrcpO;
        \addplot[scur_line]table[x = n_rows, y = var_acc]\sluppO;
        \addplot[sos_line]table[x = n_rows, y = var_acc]\sosO;
        \addplot[icur_line]table[x = n_rows, y = var_acc]\IluppTw;
        \addplot[qr_line]table[x = n_rows, y = var_acc]\IqrcpTw;
        \addplot[os_line]table[x = n_rows, y = var_acc]\IosTw;
        %\legend{\svds, \curs, \icurl};
    \end{axis}

            \begin{axis}[
        at={(axis3.outer north east)},
        anchor=outer north west,
         ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Median Accuracy Block Size 40},
        ymode = log,
        ymajorgrids,
        legend pos = south east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[sqr_line]table[x = n_rows, y = var_acc]\sqrcpO;
        \addplot[scur_line]table[x = n_rows, y = var_acc]\sluppO;
        \addplot[sos_line]table[x = n_rows, y = var_acc]\sosO;
        \addplot[icur_line]table[x = n_rows, y = var_acc]\IluppFe;
        \addplot[qr_line]table[x = n_rows, y = var_acc]\IqrcpFe;
        \addplot[os_line]table[x = n_rows, y = var_acc]\IosFe;
        %\legend{\svds, \curs, \icurl};
    \end{axis}
\end{tikzpicture}

==> plots/selection_methods/chan_1000.tex <==
\begin{tikzpicture}[scale = \boxplotscale]
    \newcommand{\matname}{Chan}
    \newcommand{\Matname}{\textsc{Chan} }
    \pgfplotstableread[col sep=comma]{./csvs/selection_methods/\matname_1000_50_med.csv}\accdata
    
    \begin{axis}[
        name = axis1,
        ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Index Selection for \Matname},
        ymode = log,
        ymajorgrids,
        legend pos = south west,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[svd_line]table[x = rank, y = svd]\accdata;
        \addplot[svds_line]table[x = rank, y = svds]\accdata;
        \addplot[qr_line]table[x = rank, y = qr]\accdata;
        \addplot[icur_line]table[x = rank, y = lupp]\accdata;
        \addplot[os_line]table[x = rank, y = os]\accdata;
        \legend{SVD, \svds, QRCP, LUPP, Osinsky};
    \end{axis}
\end{tikzpicture}

==> plots/selection_methods/circul_1000.tex <==
\begin{tikzpicture}[scale = \boxplotscale]
    \newcommand{\matname}{circul}
    \newcommand{\Matname}{\textsc{Circulent} }
    \pgfplotstableread[col sep=comma]{./csvs/selection_methods/\matname_1000_50_med.csv}\accdata
    
    \begin{axis}[
        name = axis1,
        ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Index Selection for \Matname},
        ymode = log,
        ymajorgrids,
        legend pos = south west,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[svd_line]table[x = rank, y = svd]\accdata;
        \addplot[svds_line]table[x = rank, y = svds]\accdata;
        \addplot[qr_line]table[x = rank, y = qr]\accdata;
        \addplot[icur_line]table[x = rank, y = lupp]\accdata;
        \addplot[os_line]table[x = rank, y = os]\accdata;
        \legend{SVD, \svds, QRCP, LUPP, Osinsky};
    \end{axis}
\end{tikzpicture}

==> plots/selection_methods/randsvd_6000_250.tex <==
\begin{tikzpicture}[scale = \boxplotscale]
    \newcommand{\matname}{randsvd}
    \newcommand{\Matname}{\textsc{RandSVD} }
    \pgfplotstableread[col sep=comma]{./csvs/selection_methods/\matname_6000_250_clean.csv}\accdata
    
    \begin{axis}[
        name = axis1,
        ylabel = {$\frac{\|A - \hat{A}_k\|_F}{\|A\|_F}$},
        xlabel = {Rank of Approximation},
        title = {Index Selection for \Matname},
        ymode = log,
        ymajorgrids,
        legend pos = north east,
        scale only axis,
        xlabel near ticks,
        ylabel near ticks,
        ]
        \addplot[svd_line]table[x = rank, y = svd]\accdata;
        \addplot[svds_line]table[x = rank, y = svds]\accdata;
        \addplot[qr_line]table[x = rank, y = qr]\accdata;
        \addplot[icur_line]table[x = rank, y = lupp]\accdata;
        \addplot[os_line]table[x = rank, y = os]\accdata;
        \legend{SVD, \svds, QRCP, LUPP, Osinsky};
    \end{axis}
\end{tikzpicture}
